Transactional Properties of Permissioned Blockchains

Traditional distributed transaction processing (TP) systems, such as replicated databases, faced difficulties in getting wide adoption for scenarios of enterprise integration due to the level of mutual trust required. Ironically, public blockchains, which promised to solve the problem of mutual trust in collaborative processes, suffer from issues like scalability, probabilistic transaction finality, and lack of data confidentiality. To tackle these issues, permissioned blockchains were introduced as an alternative approach combining the positives of the two worlds and avoiding their drawbacks. However, no sufficient analysis has been done to emphasize their actual capabilities regarding TP. In this paper, we identify a suitable collection of TP criteria to analyze permissioned blockchains and apply them to a prominent set of these systems. Finally, we compare the derived properties and provide general conclusions.

==> conclusionAndFutureWork.tex <==
\section{Conclusion and Future Work}

==> relatedWork.tex <==
\section{Related Work}
Here we talk about the SALT paper by Stefan Tai as well as the paper \enquote{Blockchain Consensus Protocols in the Wild}
